The Memory-Enhanced Gaussian Noise (MEGN) Model for Fiber-Optic Channels

The enhanced Gaussian noise (EGN) model is widely used for estimating the nonlinear interference (NLI) power accumulated in coherent fiber-optic transmission systems. Given a fixed fiber link, under the assumption that transmitted symbols are independent and identically distributed (i.i.d.), the EGN model establishes that the NLI power depends on time-invariant signal statistics, i.e., the second-, fourth-, and sixth-order moments of the symbols, which are determined by the modulation format and its probability distribution. However, recent advances in coded modulation have sought to mitigate NLI by introducing controlled temporal correlations among transmitted symbols, thereby violating the i.i.d. assumption underlying the EGN model. Among these correlations, symbol energy correlations are believed to exert the most significant influence on NLI. This work presents a rigorous mathematical derivation of a memory extension of the EGN model that explicitly accounts for symbol energy correlations, referred to as the MEGN model. The proposed MEGN model is validated through both numerical simulations and transmission experiments. Normalized average NLI power estimations with less than 5% errors across a wide range of symbol rates and transmission distances are reported. The model also provides a theoretical framework for analyzing and optimizing optical transmission systems employing temporally correlated modulation schemes.

==> Tex/Ch_Smart_Guards.tex <==
To suppress NLI, we exploit the co-propagating dimensions to transmit correlated symbols which are meaningless but can reduce the NLI of channel of interests (CUT).

1. Frequency: Co-propagating WDM channel with correlated data to protect the CUT.
2. Frequency: The guard interval now has non-zero spectrum where we also transmit correlated data.
3. Polarization: For IM/DD systems using only one polarization, we also transmit correlated data.

How to design the correlated data? How much gains and costs? 

==> Tex/Tab_Contribution.tex <==
\begin{table}[!t]
\centering
\caption{Break Down of Symbol-Level Energy Dependent Statistics. $\w_1\neq\w_2,\w_1\neq\w_3,\w_2\neq\w_3$} 
\label{Tab:Contributions1}
\resizebox{0.75\columnwidth}{!}{% To shrink the table
\begin{tabular}{|c|c|c|c| }
\hline
Pol. & \multirow{2}{*}{\backslashbox[55mm]{  Frequency}{Time}} & \multicolumn{2}{c|}{Double Groups Correlation}  \\ \cline{3-4}

Corr. &  & Index Subset & Moment \\ \hline
  
Intra.& $\Exp{v_{x,m} v^*_{x,n} v_{x,k} v^*_{x,m'} v_{x,n'} v^*_{x,k'}}$ & $\mLa$ & $\Exp{|\axw{1}|^4|\axw{2}|^2}$     \\ \hline
  
\multirow{4}{*}{Inter.} & $\Exp{v_{x,m} v^*_{x,n} v_{x,k} v^*_{x,m'}   v_{y,n'} v^*_{y,k'} }$ &  $\mLai{9}$ & \multirow{2}{*}{$\Exp{|\axw{1}|^4|\ayw{2}|^2}$}   \\ \cline{2-3}  

 
& $\Exp{v_{x,m} v^*_{x,m'} v_{x,n'} v^*_{x,k'}  v^*_{y,n} v_{y,k} }$ & $\mLai{4}$ &       \\ \cline{2-4}
 
& $\Exp{v_{x,m} v^*_{x,m'}  v^*_{y,n} v_{y,k}  v_{y,n'} v^*_{y,k'}}$ & $\mLai{2}$ & $\Exp{|\ayw{1}|^4|\axw{2}|^2}$        \\ \hline

\end{tabular}
}
\end{table}

==> Tex/Tab_Contribution2.tex <==
 
\begin{table}[!t]
\centering
\caption{Break Down of Symbol-Level Energy Dependent Statistics. $\w_1\neq\w_2,\w_1\neq\w_3,\w_2\neq\w_3$} 
\label{Tab:Contributions2}
\resizebox{1\columnwidth}{!}{% To shrink the table
\begin{tabular}{|c|c|c|c|c|c|}
\hline
Pol. & \multirow{2}{*}{\backslashbox[55mm]{  Frequency}{Time}} & \multicolumn{4}{c|}{Double Groups Correlation}   \\ \cline{3-6}

Corr. &  & Index Subset & Moment & Index Subset & Moment \\ \hline
  
 

Intra. & $\Exp{v_{x,m} v^*_{x,n} v_{x,k} v^*_{x,m'} v_{x,n'} v^*_{x,k'}}$  & $\mLa$ & $\Exp{\axw{1}^2\axw{2}^{*2} |\axw{2}|^2}$  & $\mLa$ & $\Exp{\axw{1}^{*2} \axw{2}^2 |\axw{2}|^2}$  \\ \hline 
  
\multirow{4}{*}{Inter.} & $\Exp{v_{x,m} v^*_{x,n} v_{x,k} v^*_{x,m'}   v_{y,n'} v^*_{y,k'} }$ &  $\mLai{9}$ & \multirow{2}{*}{$\Exp{\axw{1}^2\axw{2}^{*2} |\ayw{2}|^2}$}  & $\{\mLbi{1},\mLbi{3}\}$ & \multirow{2}{*}{$\Exp{\axw{1}^{*2} \axw{2}^2 |\ayw{2}|^2}$}   \\ \cline{2-3} \cline{5-5}

 
& $\Exp{v_{x,m} v^*_{x,m'} v_{x,n'} v^*_{x,k'}  v^*_{y,n} v_{y,k} }$ & $\mLai{4}$ &    & $\{\mLbi{3},\mLbi{4}\}$ &     \\ \cline{2-6}
 
& $\Exp{v_{x,m} v^*_{x,m'}  v^*_{y,n} v_{y,k}  v_{y,n'} v^*_{y,k'}}$ & $\mLai{2}$ & $\Exp{\ayw{1}^2\ayw{2}^{*2} |\axw{2}|^2}$   &   $\{\mLbi{3},\mLbi{5}\}$ & $\Exp{\ayw{1}^{*2} \ayw{2}^2 |\axw{2}|^2}$  \\ \hline

\end{tabular}
}
\end{table}



==> Tex/Tab_Contribution3.tex <==
 
\begin{table}[!t]
\centering
\caption{Break Down of Symbol-Level Energy Dependent Statistics. $\w_1\neq\w_2,\w_1\neq\w_3,\w_2\neq\w_3$} 
\label{Tab:Contributions3}
\resizebox{0.75\columnwidth}{!}{% To shrink the table
\begin{tabular}{|c|c|c|c| }
\hline
Pol. & \multirow{2}{*}{\backslashbox[55mm]{  Frequency}{Time}} & \multicolumn{2}{c|}{Triple Groups Correlation}   \\ \cline{3-4}

Corr. &  & Index Subset & Moment  \\ \hline

Intra. & $\Exp{v_{x,m} v^*_{x,n} v_{x,k} v^*_{x,m'} v_{x,n'} v^*_{x,k'}}$  & $\mLa$ & $\Exp{\axw{1}^2\axw{2}^{*2} |\axw{3}|^2}$   \\ \hline 
  
\multirow{4}{*}{Inter.} & $\Exp{v_{x,m} v^*_{x,n} v_{x,k} v^*_{x,m'}   v_{y,n'} v^*_{y,k'} }$ &  $\mLai{9}$ & \multirow{2}{*}{$\Exp{\axw{1}^2\axw{2}^{*2} |\ayw{3}|^2}$}      \\ \cline{2-3}  
 
& $\Exp{v_{x,m} v^*_{x,m'} v_{x,n'} v^*_{x,k'}  v^*_{y,n} v_{y,k} }$ & $\mLai{4}$   &  \\ \cline{2-4}
 
& $\Exp{v_{x,m} v^*_{x,m'}  v^*_{y,n} v_{y,k}  v_{y,n'} v^*_{y,k'}}$ & $\mLai{2}$ & $\Exp{\ayw{1}^2\ayw{2}^{*2} |\axw{3}|^2}$    \\ \hline

\end{tabular}
}
\end{table}



==> Tex/Tab_Contribution4.tex <==
\begin{table}[!t]
\centering
\caption{Break Down of Symbol-Level Energy Dependent Statistics. $\w_1\neq\w_2,\w_1\neq\w_3,\w_2\neq\w_3$} 
\label{Tab:Contributions4}
\resizebox{0.75\columnwidth}{!}{% To shrink the table
\begin{tabular}{|c|c|c|c| }
\hline
Pol. & \multirow{2}{*}{\backslashbox[55mm]{  Frequency}{Time}} & \multicolumn{2}{c|}{Triple Groups Correlation} \\ \cline{3-4}

Corr. &  & Index Subset & Moment  \\ \hline
  
Intra.& $\Exp{v_{x,m} v^*_{x,n} v_{x,k} v^*_{x,m'} v_{x,n'} v^*_{x,k'}}$ & $\mLb$ & $\Exp{|\axw{1}|^2|\axw{2}|^2|\axw{3}|^2}$   \\ \hline
  
\multirow{4}{*}{Inter.} & $\Exp{v_{x,m} v^*_{x,n} v_{x,k} v^*_{x,m'}   v_{y,n'} v^*_{y,k'} }$  & $\{\mLbi{1},\mLbi{3}\}$ & \multirow{2}{*}{$\Exp{|\axw{1}|^2|\axw{2}|^2|\ayw{3}|^2}$}   \\ \cline{2-3}  

 
& $\Exp{v_{x,m} v^*_{x,m'} v_{x,n'} v^*_{x,k'}  v^*_{y,n} v_{y,k} }$  & $\{\mLbi{3},\mLbi{4}\}$ &     \\ \cline{2-4}
 
& $\Exp{v_{x,m} v^*_{x,m'}  v^*_{y,n} v_{y,k}  v_{y,n'} v^*_{y,k'}}$  &   $\{\mLbi{3},\mLbi{5}\}$ & $\Exp{|\axw{1}|^2|\ayw{2}|^2|\ayw{3}|^2}$  \\ \hline

\end{tabular}
}
\end{table}

==> Tex/Tab_Correction_Terms222.tex <==

\begin{table}[ht]
\centering
\caption{The $\Lambda_i$ and $\Xi_i$ used in the Correction Terms.}
\resizebox{0.8\columnwidth}{!}{ 
\begin{tabular}{|c|c c| c c|}
\hline
& Name & Value & Name & Value \\ \hline 

\multirow{13}{*}{$\mLb^{a}$} & $\xi_1$ & 4 & $\Xi^a_1$ & $\exp{\left(-\jmath\frac{2\pi}{R_s}\tau_1(f-f_1)\right)}+\exp{\left(-\jmath\frac{2\pi}{R_s}\tau_2(f-f_1)\right)}$   \\ \cline{2-5}
& $\xi_2$ & $-4$ & $\Xi^a_2$ & $ \exp{\left(-\jmath\frac{2\pi}{R_s} \tau_1 (f-f_1)\right)} $   \\ \cline{2-5}
& $\xi_3$ & $-4$ & $\Xi^a_3$ & $ \exp{\left(-\jmath\frac{2\pi}{R_s} \tau_2 (f-f_1)\right)} $   \\ \cline{2-5}
& $\xi_4$ & 4& $\Xi^a_4$ & $\exp{\left(-\jmath\frac{2\pi}{R_s}\tau_1(f_1-f)\right)}+\exp{\left(-\jmath\frac{2\pi}{R_s}(\tau_2-\tau_1)(f-f_1)\right)}$   \\ \cline{2-5}
& $\xi_5$ & $-4$ & $\Xi^a_5$ & $ \exp{\left(-\jmath\frac{2\pi}{R_s} \tau_1 (f_1-f)\right)} $   \\ \cline{2-5}
& $\xi_6$ & $-4$ & $\Xi^a_6$ & $ \exp{\left(-\jmath\frac{2\pi}{R_s} (\tau_2-\tau_1) (f-f_1)\right)} $   \\ \cline{2-5}
& $\xi_7$ & 4 & $\Xi^a_7$ & $\exp{\left(-\jmath\frac{2\pi}{R_s}(\tau_1-\tau_2)(f-f_1)\right)}+\exp{\left(-\jmath\frac{2\pi}{R_s}\tau_2(f_1-f)\right)}$   \\ \cline{2-5}
& $\xi_8$ & $-4$ & $\Xi^a_8$ & $ \exp{\left(-\jmath\frac{2\pi}{R_s} (\tau_1-\tau_2) (f-f_1)\right)} $   \\ \cline{2-5}
& $\xi_9$ & $-4$ & $\Xi^a_9$ & $ \exp{\left(-\jmath\frac{2\pi}{R_s} \tau_2 (f_1-f)\right)} $   \\ \hline \hline

\multirow{9}{*}{$\mLb^{b}$} & $\xi_{10}$ & 2 & $\Xi^b_{1}$ & $ \exp{\left(-\jmath\frac{2\pi}{R_s} (\tau_1 f_1 + \tau_2 f_2)\right)} $   \\ \cline{2-5}
& $\xi_{11}$ & 2 & $\Xi^b_{2}$ & $ \exp{\left(-\jmath\frac{2\pi}{R_s} (\tau_2 f_1 + \tau_1 f_2)\right)} $   \\ \cline{2-5}
& $\xi_{12}$ & 2 & $\Xi^b_{3}$ & $ \exp{\left(-\jmath\frac{2\pi}{R_s} (-\tau_1 f_1 + (\tau_2-\tau_1) f_2)\right)} $   \\ \cline{2-5}
& $\xi_{13}$ & 2 & $\Xi^b_{4}$ & $ \exp{\left(-\jmath\frac{2\pi}{R_s} ((\tau_2-\tau_1) f_1-\tau_1 f_2  )\right)} $   \\ \cline{2-5}
& $\xi_{14}$ & 2 & $\Xi^b_{5}$ & $ \exp{\left(-\jmath\frac{2\pi}{R_s} ((\tau_1-\tau_2) f_1-\tau_2 f_2  )\right)} $   \\ \cline{2-5}
& $\xi_{15}$ & 2  & $\Xi^b_{6}$ & $ \exp{\left(-\jmath\frac{2\pi}{R_s} (-\tau_2 f_1+  (\tau_1-\tau_2) f_2)\right)} $   \\ \hline

\end{tabular}
}
\end{table}
 

==> Tex/Tab_Correction_Terms222A.tex <==

\begin{table}[ht]
\centering
\caption{The $\Lambda_i$ and $\Xi_i$ used in the Correction Terms.}
\resizebox{0.8\columnwidth}{!}{ 
\begin{tabular}{|lc|lc|  }
\hline
\multicolumn{1}{|c }{\textbf{Name}} & \multicolumn{1}{ c|}{\textbf{Value}} & \multicolumn{1}{|c }{\textbf{Name}} & \multicolumn{1}{ c|}{\textbf{Value}}  \\ \hline 

$\xi_1$ & 1 & $\Xi_1$ & $\exp{\left(-\jmath\frac{2\pi}{R_s}\tau_1(f_1+f_2)\right)}+\exp{\left(-\jmath\frac{2\pi}{R_s}\tau_2(f_1+f_2)\right)}$   \\ \hline
$\xi_2$ & $-1$ & $\Xi_2$ & $ \exp{\left(-\jmath\frac{2\pi}{R_s}\tau_1(f_1+f_2)\right)} $   \\ \hline
$\xi_3$ & $-1$ & $\Xi_3$ & $\exp{\left(-\jmath\frac{2\pi}{R_s}\tau_2(f_1+f_2)\right)} $   \\ \hline\hline 

$\xi_4$ & 1& $\Xi_4$ & $\exp{\left(-\jmath\frac{2\pi}{R_s}(-\tau_1)(f_1+f_2)\right)}+\exp{\left(-\jmath\frac{2\pi}{R_s}(\tau_2-\tau_1)(f_1+f_2)\right)}$   \\ \hline
$\xi_5$ & $-1$ & $\Xi_5$ & $ \exp{\left(-\jmath\frac{2\pi}{R_s}(-\tau_1)(f_1+f_2)\right)} $   \\ \hline  
$\xi_6$ & $-1$ & $\Xi_6$ & $ \exp{\left(-\jmath\frac{2\pi}{R_s}(\tau_2-\tau_1)(f_1+f_2)\right)} $   \\ \hline\hline 

$\xi_7$ & 1 & $\Xi_7$ & $\exp{\left(-\jmath\frac{2\pi}{R_s}(\tau_1-\tau_2)(f_1+f_2)\right)}+\exp{\left(-\jmath\frac{2\pi}{R_s}( -\tau_2)(f_1+f_2)\right)}$  \\ \hline
$\xi_8$ & $-1$ & $\Xi_8$ & $ \exp{\left(-\jmath\frac{2\pi}{R_s}(\tau_1-\tau_2)(f_1+f_2)\right)} $   \\ \hline
$\xi_9$ & $-1$ & $\Xi_9$ & $ \exp{\left(-\jmath\frac{2\pi}{R_s}( -\tau_2)(f_1+f_2)\right)}$   \\ \hline \hline

$\xi_{10}$ & 2 & $\Xi_{10}$ & $\exp{\left(-\jmath\frac{2\pi}{R_s}\tau_1 (f_1+f_2)\right)}+\exp{\left(-\jmath\frac{2\pi}{R_s} \tau_2 (f-f_1)\right)}$  \\ \hline
$\xi_{11}$ & $-2$ & $\Xi_{11}$ & $\exp{\left(-\jmath\frac{2\pi}{R_s}\tau_1 (f_1+f_2)\right)} $   \\ \hline
$\xi_{12}$ & $-2$ & $\Xi_{12}$ & $\exp{\left(-\jmath\frac{2\pi}{R_s} \tau_2 (f-f_1)\right)}$   \\ \hline \hline

$\xi_{13}$ & 2 & $\Xi_{13}$ & $\exp{\left(-\jmath\frac{2\pi}{R_s}\tau_2 (f_1+f_2)\right)}+\exp{\left(-\jmath\frac{2\pi}{R_s} \tau_1 (f-f_1)\right)}$  \\ \hline
$\xi_{14}$ & $-2$ & $\Xi_{14}$ & $\exp{\left(-\jmath\frac{2\pi}{R_s}\tau_2 (f_1+f_2)\right)} $   \\ \hline
$\xi_{15}$ & $-2$ & $\Xi_{15}$ & $\exp{\left(-\jmath\frac{2\pi}{R_s} \tau_1 (f-f_1)\right)}$   \\ \hline \hline

$\xi_{16}$ & 2 & $\Xi_{16}$ & $\exp{\left(-\jmath\frac{2\pi}{R_s}(-\tau_1) (f_1+f_2)\right)}+\exp{\left(-\jmath\frac{2\pi}{R_s} (\tau_2-\tau_1) (f-f_1)\right)}$  \\ \hline
$\xi_{17}$ & $-2$ & $\Xi_{17}$ & $\exp{\left(-\jmath\frac{2\pi}{R_s}(-\tau_1) (f_1+f_2)\right)} $   \\ \hline
$\xi_{18}$ & $-2$ & $\Xi_{18}$ & $\exp{\left(-\jmath\frac{2\pi}{R_s} (\tau_2-\tau_1) (f-f_1)\right)}$   \\ \hline \hline

$\xi_{19}$ & 2 & $\Xi_{19}$ & $\exp{\left(-\jmath\frac{2\pi}{R_s}(\tau_2-\tau_1) (f_1+f_2)\right)}+\exp{\left(-\jmath\frac{2\pi}{R_s} ( -\tau_1) (f-f_1)\right)}$  \\ \hline
$\xi_{20}$ & $-2$ & $\Xi_{20}$ & $\exp{\left(-\jmath\frac{2\pi}{R_s}(\tau_2-\tau_1) (f_1+f_2)\right)} $   \\ \hline
$\xi_{21}$ & $-2$ & $\Xi_{21}$ & $\exp{\left(-\jmath\frac{2\pi}{R_s} (-\tau_1) (f-f_1)\right)}$   \\ \hline \hline

$\xi_{22}$ & 2 & $\Xi_{22}$ & $\exp{\left(-\jmath\frac{2\pi}{R_s}(\tau_1-\tau_2) (f_1+f_2)\right)}+\exp{\left(-\jmath\frac{2\pi}{R_s} ( -\tau_2) (f-f_1)\right)}$  \\ \hline
$\xi_{23}$ & $-2$ & $\Xi_{23}$ & $\exp{\left(-\jmath\frac{2\pi}{R_s}(\tau_1-\tau_2) (f_1+f_2)\right)} $   \\ \hline
$\xi_{24}$ & $-2$ & $\Xi_{24}$ & $\exp{\left(-\jmath\frac{2\pi}{R_s} (-\tau_2) (f-f_1)\right)}$   \\ \hline \hline

$\xi_{25}$ & 2 & $\Xi_{25}$ & $\exp{\left(-\jmath\frac{2\pi}{R_s}(-\tau_2) (f_1+f_2)\right)}+\exp{\left(-\jmath\frac{2\pi}{R_s} (\tau_1 -\tau_2) (f-f_1)\right)}$  \\ \hline
$\xi_{26}$ & $-2$ & $\Xi_{26}$ & $\exp{\left(-\jmath\frac{2\pi}{R_s}(-\tau_2) (f_1+f_2)\right)} $   \\ \hline
$\xi_{27}$ & $-2$ & $\Xi_{27}$ & $\exp{\left(-\jmath\frac{2\pi}{R_s} (\tau_1-\tau_2) (f-f_1)\right)}$   \\ \hline \hline

$\xi_{28}$ & 4 & $\Xi_{28}$ & $\exp{\left(-\jmath\frac{2\pi}{R_s}\left((\tau_1-\tau_2)f_1+ \tau_2(f-f_2)\right)\right)}+\exp{\left(-\jmath\frac{2\pi}{R_s} (\tau_2 -\tau_1) f_1 + \tau_1(f-f_2)\right)}$  \\ \hline
$\xi_{29}$ & $-4$ & $\Xi_{29}$ & $\exp{\left(-\jmath\frac{2\pi}{R_s}\left((\tau_1-\tau_2)f_1+ \tau_2(f-f_2)\right)\right)} $   \\ \hline
$\xi_{30}$ & $-4$ & $\Xi_{30}$ & $\exp{\left(-\jmath\frac{2\pi}{R_s} (\tau_2 -\tau_1) f_1 + \tau_1(f-f_2)\right)}$   \\ \hline \hline

$\xi_{31}$ & 4 & $\Xi_{31}$ & $\exp{\left(-\jmath\frac{2\pi}{R_s}\left((-\tau_2)f_1+ (\tau_1-\tau_2)(f_2-f)\right)\right)}+\exp{\left(-\jmath\frac{2\pi}{R_s} ( -\tau_2) f_1 + \tau_1(f_2-f)\right)}$  \\ \hline
$\xi_{32}$ & $-4$ & $\Xi_{32}$ & $\exp{\left(-\jmath\frac{2\pi}{R_s}\left((-\tau_2)f_1+ (\tau_1-\tau_2)(f_2-f)\right)\right)} $   \\ \hline
$\xi_{33}$ & $-4$ & $\Xi_{33}$ & $\exp{\left(-\jmath\frac{2\pi}{R_s} ( -\tau_2) f_1 + \tau_1(f_2-f)\right)}$   \\ \hline \hline

$\xi_{34}$ & 4 & $\Xi_{34}$ & $\exp{\left(-\jmath\frac{2\pi}{R_s}\left( \tau_1 f_1+  \tau_2 (f_2-f)\right)\right)}+\exp{\left(-\jmath\frac{2\pi}{R_s} ( -\tau_1) f_1 + (\tau_2 -\tau_1)(f_2-f)\right)}$  \\ \hline
$\xi_{35}$ & $-4$ & $\Xi_{35}$ & $\exp{\left(-\jmath\frac{2\pi}{R_s}\left( \tau_1 f_1+  \tau_2 (f_2-f)\right)\right)}$   \\ \hline
$\xi_{36}$ & $-4$ & $\Xi_{36}$ & $\exp{\left(-\jmath\frac{2\pi}{R_s} ( -\tau_1) f_1 + (\tau_2 -\tau_1)(f_2-f)\right)}$   \\ \hline \hline



\end{tabular}
}
\end{table}
 

==> Tex/Tab_Correction_Terms24.tex <==
 
\begin{table}[ht]
\centering
\caption{The $\Lambda_i$ and $\Xi_i$ used in the Correction Terms.}
\resizebox{0.55\columnwidth}{!}{  
% \begin{tabular}{|lc|lc|lc|}
% \hline
% \multicolumn{1}{|c }{\textbf{Name}} & \multicolumn{1}{ c|}{\textbf{Value}}& \multicolumn{1}{|c }{\textbf{Name}} & \multicolumn{1}{ c|}{\textbf{Value}} & \multicolumn{1}{|c }{\textbf{Name}} & \multicolumn{1}{ c|}{\textbf{Value}}\\ \hline
 
% $\Lambda_1$ & $2\cos{\left(\frac{2\pi}{R_s}\tau f_1  \right)}$ & $\Lambda_3$ & $2\cos^2{\left(\frac{\pi}{R_s}\tau(f_1-f)\right)}$ &  $\Lambda_5$ &  1 \\ \hline
% $\Lambda_2$ & $2\sin{\left(\frac{2\pi}{R_s}\tau f_1  \right)}$  & $\Lambda_4$ & $2\jmath\sin^2{\left(\frac{\pi}{R_s}\tau(f_1-f)\right)}$  &  \multicolumn{2}{c|}{---}  \\\hline
 
% \end{tabular}
\begin{tabular}{|c|c c| c c|}
\hline
& Name & Value & Name & Value \\ \hline
$\mLa^{c}$ &  $\lambda_1$ & 2 & $\Lambda^c_1$ & 1 \\ \hline
\multirow{2}{*}{$\mLa^{b}$} & $\lambda_2$ & 8 & $\Lambda^b_1$ & $\cos{\left(\frac{2\pi}{R_s}\tau f_1  \right)}$ \\ \cline{2-5}
 & $\lambda_3$ & 8 & $\Lambda^b_2$ & $\sin{\left(\frac{2\pi}{R_s}\tau f_1  \right)}$  \\ \hline \hline
\multirow{2}{*}{$\mLa^{a}$} & $\lambda_4$ & 8 & $\Lambda^a_1$ & $\cos^2{\left(\frac{\pi}{R_s}\tau(f_1-f)\right)}$ \\ \cline{2-5}
& $\lambda_5$ & $-8$ & $\Lambda^a_2$ & $\sin^2{\left(\frac{\pi}{R_s}\tau(f_1-f)\right)}$  \\ \hline
 
\end{tabular}
}
\end{table}



==> Tex/Tab_Correction_Terms24A.tex <==
 
\begin{table}[ht]
\centering
\caption{The $\Lambda_i$ and $\Xi_i$ used in the Correction Terms.}
\resizebox{0.55\columnwidth}{!}{   

\begin{tabular}{|lc|lc|}
\hline
\multicolumn{1}{|c }{\textbf{Name}} & \multicolumn{1}{ c|}{\textbf{Value}}& \multicolumn{1}{|c }{\textbf{Name}} & \multicolumn{1}{ c|}{\textbf{Value}}\\ \hline
$\lambda_1$ & 4 & $\Lambda_1$ & $\cos^2{\left(\frac{\pi}{R_s}\tau(f_1+f_2)\right)}$ \\ \hline
$\lambda_2$ & $-4$ & $\Lambda_2$ &  $\sin^2{\left(\frac{\pi}{R_s}\tau(f_1+f_2)\right)}$ \\ \hline  \hline
$\lambda_3$ & 8 & $\Lambda_3$ & $\cos{\left(\frac{\pi}{R_s}\tau (2f_1+f_2-f)  \right) } \cos{\left(\frac{\pi}{R_s}\tau (f-f_2)  \right) }$  \\ \hline
$\lambda_4$ &  $-8$ & $\Lambda_4$ & $\cos{\left(\frac{\pi}{R_s}\tau (2f_1+f_2-f)  \right) } \sin{\left(\frac{\pi}{R_s}\tau (f-f_2)  \right) }$ \\ \hline
$\lambda_5$ & $8$ & $\Lambda_5$ & $\sin{\left(\frac{\pi}{R_s}\tau (2f_1+f_2-f)  \right) } \cos{\left(\frac{\pi}{R_s}\tau (f-f_2)  \right) }$  \\ \hline
$\lambda_6$ & $-8$ & $\Lambda_6$ & $\sin{\left(\frac{\pi}{R_s}\tau (2f_1+f_2-f)  \right) } \sin{\left(\frac{\pi}{R_s}\tau (f-f_2)  \right) }$  \\ \hline
 
\end{tabular}
}
\end{table}



==> Tex/Tab_Model_Assumption.tex <==
 
\begin{table*}[ht]
\centering 
\caption{Comparison of signaling assumptions of NLI power models. } 
\label{Tab:Symbol_Statistics_Overview}
\resizebox{0.8\textwidth}{!}{% To shrink the table
\begin{tabular}{|c|c|c|c|c|}
\hline
\multirow{2}{*}{\textbf{Dependency}} & \multicolumn{4}{c|}{\textbf{Models}} \\
\cline{2-5}
 & GN & EGN  & 4D EGN & This work: FEGN \\
\hline
Frequency Tones & $\times$ & $\checkmark$ & $\checkmark$ & $\checkmark$ \\ \hline
% I/Q Components & $\times$ & $\times$ & $\checkmark$ & $\checkmark$ \\
Polarizations & $\times$ & $\times$ & $\checkmark$ & $\checkmark$ \\ \hline 
Time  & $\times$ & $\times$ & $\times$ & $\checkmark$ \\ \hline
\multirow{5}{*}{\textbf{Signal Statistics }}  & \multicolumn{3}{c|}{Modulation  } & 4D modulation with temporal correlation, e.g.,  $\Exp{|a_{x,i}|^2|a_{y,j}|^4}$\\ \cline{4-5}
&     \multicolumn{2}{c|}{Dependent  } &\multicolumn{2}{c|}{4D modulation with cross-pol. correlation, e.g., $\Exp{|a_x|^2 |a_y|^4}$}  \\ \cline{3-5}
& Statistics & \multicolumn{3}{c|}{2D modulation format's 4/6-th order moments, e.g., $\Exp{|a|^2}\Exp{|a|^4}$}  \\ \cline{2-5}
 &  \multicolumn{4}{c|}{Cube of average power $\Exp{|a|^2}^3$} \\ \hline


\end{tabular}}
\end{table*}

% \begin{table}[ht]
% \centering
% \caption{Comparison of signaling assumptions of EGN models. } 
% \label{Tab:Assumptions}
% \renewcommand{\arraystretch}{1.5}
% \resizebox{0.8\columnwidth}{!}{% To shrink the table
% % \setlength{\tabcolsep}{6pt}
% \begin{tabular}{|c|c||c|c|c|}
% \hline 
% \multicolumn{2}{|c||}{\textbf{Signaling Assumption}}   & \textbf{EGN} & \textbf{4D EGN (G. Liga)} & \textbf{This Work} \\ \hline 
% I/Q Dim. &Zero Mean \& Symmetric  & \multicolumn{3}{|c|}{Yes}  \\ \hline
% \multirow{2}{*}{Pol. Dim.} & Pol. Distribution & Identical & Arbitrary & Arbitrary \\ \cline{2-5}
%  & Pol. Dependency & Independent & Arbitrary & Arbitrary \\ \hline
% \multirow{2}{*}{Time Dim.} & Amplitude (Energy) & i.i.d. & i.i.d. & Arbitrary \\ \cline{2-5}
%  & Phase & i.i.d. & Arbitrary & i.i.d. \\ \hline
% \end{tabular}
% }
% \end{table}
 


==> Tex/Tab_Subsets1.tex <==
%%% Table correlation contribution
\begin{table} 
    \caption{The Categorization of the Symbol-Level Energy Dependent Statistics. }
    \centering
    \label{Tab:Statis}
    \resizebox{0.7\columnwidth}{!}{% To shrink the table
    \begin{tabular}{|c|c|c| } 
\hline 
Number of Delays & Subsets & Energy Dependent  \\
\hline 
0 & $ \w_1=\w_2=\ldots=\w_6 $ & $\Exp{|\axw{1}|^6}$  \\ 

1 & $\mLa$ & $\Exp{|\axw{1}|^4|\axw{2}|^2}$  \\ 

2 & $\mLb$ & $\Exp{|\axw{1}|^2|\axw{2}|^2|\axw{3}|^2}$  \\
 
\hline
\end{tabular}
}
\end{table}


% %%% Table correlation contribution
% \begin{table} 
%     \caption{The Categorization of the Symbol-Level Energy Dependent Statistics. }
%     \centering
%     \label{Tab:Statis}
%     \resizebox{1\columnwidth}{!}{% To shrink the table
%     \begin{tabular}{|c|c|c| } 
% \hline 
% Number of Delays & Subsets & Energy Dependent  \\
% \hline 
% 0 & $\mL_0=\{\bomega\in\mL:\w_1=\w_2=\w_3=\w_4=\w_5=\w_6\}$ & $\Exp{|\axw{1}|^6}$  \\ 

% 1 & $\mL_2=\{\bomega\in\mL:\w_{k_1}=\w_{k_2}=\w_{k_3}=\w_{k_4},\w_{k_5}=\w_{k_6},\w_{k_1}\neq\w_{k_5}\}$ & $\Exp{|\axw{1}|^4|\axw{2}|^2}$  \\ 

% 2 & $\mL_2=\{\bomega\in\mL:\w_{k_1}=\w_{k_2},\w_{k_3}=\w_{k_4},\w_{k_5}=\w_{k_6},\w_{k_1}\neq\w_{k_3}\neq\w_{k_5}\}$ & $\Exp{|\axw{1}|^2|\axw{2}|^2|\axw{3}|^2}$  \\
 
% \hline
% \end{tabular}
% }
% \end{table}

% %%% Table correlation contribution
% \begin{table} 
%     \caption{The categorization of the symbol-level signal statistics. $k_i \in \{1, 2, \ldots,6\},k_i \neq k_j, \forall \, i \neq j $}
%     \centering
%     \label{Tab:Statis}
%     \resizebox{1\columnwidth}{!}{% To shrink the table
%     \begin{tabular}{|c|c|c|c|} 
% \hline 
% Number of Delays & Subsets & Energy Dependent & sign dependent \\
% \hline 
% 1 & $\mL_1=\{\bomega\in\mL:\w_1=\w_2=\w_3=\w_4=\w_5=\w_6\}$ & $\Exp{|\axw{1}|^6}$ & - \\

% 2 & $\mL_2=\{\bomega\in\mL:\w_{k_1}=\w_{k_2}=\w_{k_3}=\w_{k_4}=\w_{k_5},\w_{k_1}\neq\w_{k_6}\}$ &- & $\Exp{|\axw{1}|^4\axw{1}\axw{2}^*}$  \\

% 2 & $\mL_2=\{\bomega\in\mL:\w_{k_1}=\w_{k_2}=\w_{k_3},\w_{k_4}=\w_{k_5}=\w_{k_6},\w_{k_1}\neq\w_{k_4}\}$  & - & $\Exp{|\axw{1}|^2|\axw{2}|^2 \axw{1}\axw{2}^*}$ \\

% 2 & $\mL_2=\{\bomega\in\mL:\w_{k_1}=\w_{k_2}=\w_{k_3}=\w_{k_4},\w_{k_5}=\w_{k_6},\w_{k_1}\neq\w_{k_5}\}$ & $\Exp{|\axw{1}|^4|\axw{2}|^2}$ & - \\

% 3 & $\mL_2=\{\bomega\in\mL:\w_{k_1}=\w_{k_2}=\w_{k_3}=\w_{k_4},\w_{k_1}\neq\w_{k_5}\neq\w_{k_6}\}$ & - & $\Exp{|\axw{1}|^4\axw{2}\axw{3}^*}$ \\

% 3 & $\mL_2=\{\bomega\in\mL:\w_{k_1}=\w_{k_2},\w_{k_3}=\w_{k_4},\w_{k_5}=\w_{k_6},\w_{k_1}\neq\w_{k_3}\neq\w_{k_5}\}$ & $\Exp{|\axw{1}|^2|\axw{2}|^2|\axw{3}|^2}$ & - \\

% 4 & $\mL_2=\{\bomega\in\mL:\w_{k_1}=\w_{k_2}=\w_{k_3},\w_{k_3}\neq\w_{k_4}\neq\w_{k_5}\neq\w_{k_6}\}$ & - & $\Exp{|\axw{1}|^2|\axw{1} \axw{2} \axw{3} \axw{4} }$  \\

% 5 & $\mL_2=\{\bomega\in\mL:\w_{k_1}=\w_{k_2},\w_{k_2}\neq\w_{k_3}\neq\w_{k_4}\neq\w_{k_5}\neq\w_{k_6}\}$ & - & $\Exp{|\axw{1}|^2\axw{2}\axw{3}^*\axw{4}\axw{5}^*}$ \\

% 6 & $\mL_2=\{\bomega\in\mL:\w_{k_i}\neq\w_{k_j}, \forall i\neq j\}$ & -  &$\Exp{\axw{1}\axw{2}^*\axw{3}\axw{4}^*\axw{5}\axw{6}^*}$ \\
% \hline
% \end{tabular}
% }
% \end{table}

==> Tex/Tab_Subsets2.tex <==
%%% Table correlation contribution
\begin{table} 
    \caption{The Categorization of the Symbol-Level Energy Dependent Statistics. }
    \centering
    \label{Tab:Statis}
    \resizebox{0.7\columnwidth}{!}{% To shrink the table
    \begin{tabular}{|c|c|c| } 
\hline 
Number of Delays & Subsets & Energy Dependent  \\
\hline 
0 & $ \w_1=\w_2=\ldots=\w_6 $ & $\Exp{|\axw{1}|^4|\ayw{1}|^2}$  \\ 

1 & $ \mLai{4} $ & $\Exp{|\axw{1}|^4|\ayw{2}|^2}$  \\ 

2 & $\mLbi{3},\mLbi{4}$ & $\Exp{|\axw{1}|^2|\axw{2}|^2|\ayw{3}|^2}$  \\  
\hline
\end{tabular}
}
\end{table}

 

==> Tex/Tab_Subsets3.tex <==
%%% Table correlation contribution
\begin{table} 
    \caption{The Categorization of the Symbol-Level Energy Dependent Statistics. }
    \centering
    \label{Tab:Statis}
    \resizebox{0.7\columnwidth}{!}{% To shrink the table
    \begin{tabular}{|c|c|c| } 
\hline 
Number of Delays & Subsets & Energy Dependent  \\
\hline 
0 & $ \w_1=\w_2=\ldots=\w_6 $ & $\Exp{|\axw{1}|^2|\ayw{1}|^4}$  \\ 

1 & $ \mLai{2} $ & $\Exp{|\axw{1}|^2|\ayw{2}|^4}$  \\ 

2 & $\mLbi{3},\mLbi{5}$ & $\Exp{|\axw{1}|^2|\ayw{2}|^2|\ayw{3}|^2}$  \\  
\hline
\end{tabular}
}
\end{table}

 

==> Tex/Tab_SymCorrCat.tex <==

% \begin{table}[!t]
% \centering
% \caption{Symbol-Level Energy Correlations and Corresponding covariance}
% \label{Tab:MomList_1D_2D}
% \renewcommand{\arraystretch}{1.55}
% \resizebox{1\linewidth}{!}{% To ensure the table fits within the column width
% \begin{tabular}{|c|c|c|c|c|c|c|}
% \hline
% \multirow{2}{*}{Symbol Correlation} & \multicolumn{6}{c|}{Number of Index Groups} \\ \cline{2-7}
%  & $\mL_{1}$ & $\mLa^{a}$ & $\mLa^{b}$ & $\mLa^{c}$ & $\mLb^{a}$ & $\mLb^{b}$ \\ \hline 
% $ \Ka{\w,\tau}  $ &  0 & 4 & 4 & 1 &0 & 0 \\  \hline
%  $\Kb{\w,\tau,\taup}$ &  \multirow{2}{*}{0} & \multirow{2}{*}{0} & \multirow{2}{*}{0} & \multirow{2}{*}{0} & \multirow{2}{*}{4} & \multirow{2}{*}{2} \\  
%    $ \Exp{|\ax|^2}\Kc{\w,\tau} $   & & &   &  & &    \\  \hline
% \end{tabular}
% }
% \end{table}

\begin{table}[!t]
\centering
\caption{Symbol-Level Energy Correlations and Corresponding covariance }
\label{Tab:MomList_1D_2D}
\renewcommand{\arraystretch}{1.55}
\resizebox{1\linewidth}{!}{%
\begin{tabular}{|c|c|c|}
\hline
Index Group Type & \# each Type & Involved Correlations \\ \hline
$\mL_{1}$      & \multicolumn{2}{c|}{--} \\ \hline
$\mLa^{a}$     & 4 &  \multirow{3}{*}{$\bKSa{ \tau}$} \\ \cline{1-2}
$\mLa^{b}$     & 4 &  \\ \cline{1-2}
$\mLa^{c}$     & 1 & \\ \hline
$\mLb^{a}$     & 4 & $\bKSc{ \tau}$ \\ \cline{1-2}
$\mLb^{b}$     & 2 &  $\bKSb{ \tau,\taup}$ \\ \hline
\end{tabular}
}
\end{table}


% \begin{table}[!t]
% \centering
% \caption{Symbol-Level Energy Dependent Statistics for 4D Mapping}
% \label{Tab:MomList_4D}
% \renewcommand{\arraystretch}{1.55}
% \resizebox{1\linewidth}{!}{% To ensure the table fits within the column width
% \begin{tabular}{|c|c|c|c|c|c|c|}
% \hline
% \multirow{2}{*}{Symbol Correlation} & \multicolumn{6}{c|}{Number of Index Groups} \\ \cline{2-7}
%  & $\mL_{1}$ & $\mLa^{a}$ & $\mLa^{b}$ & $\mLa^{c}$ & $\mLb^{a}$ & $\mLb^{b}$ \\ \hline 
%  $\Ko $   &  2 & 0 & 0 & 0 &0 & 0 \\  \hline
% $ \Ka{\w,\tau}  $ &  0 & 6 & 5 & 1 &0 & 0 \\  \hline
% $ \Kaa{\w,\tau} $ &  0 & 6 & 5 & 1 &0 & 0 \\  \hline
%    $ \Exp{|\ax|^2}\Kc{\w,\tau} $   &  0 & 0 & 0 & 0 &9 & 3  \\  \hline
%    $\Kb{\w,\tau,\taup}$ &  0 & 0 & 0 & 0 &9 & 3 \\  \hline
% \end{tabular}
% }
% \end{table}


% \begin{table}[!t]
% \centering
% \caption{Symbol-Level Energy Correlations and Corresponding covariance }
% \label{Tab:MomList_4D}
% \renewcommand{\arraystretch}{1.55}
% \resizebox{1\linewidth}{!}{%
% \begin{tabular}{|c|c|c|}
% \hline
% Index Group Type & \# each Type & Involved Correlations \\ \hline
% $\mL_{1}$      & \multicolumn{2}{c|}{--} \\ \hline
% $\mLa^{a}$     & 4 &  \multirow{3}{*}{$\bKSa{ \tau}$} \\ \cline{1-2}
% $\mLa^{b}$     & 4 &  \\ \cline{1-2}
% $\mLa^{c}$     & 1 & \\ \hline
% $\mLb^{a}$     & 4 & $\bKSc{ \tau}$ \\ \cline{1-2}
% $\mLb^{b}$     & 2 &  $\bKSb{ \tau,\taup}$ \\ \hline
% \end{tabular}
% }
% \end{table}

==> Tex/Tab_SymCorrCat2.tex <==


\begin{table}[!t]
\centering
\caption{Symbol-Level Energy Correlations and Corresponding covariance }
\label{Tab:MomList_4D}
\renewcommand{\arraystretch}{1.55}
\resizebox{1\linewidth}{!}{%
\begin{tabular}{|c|c|c|}
\hline
Index Group Type & \# each Type & Involved Correlations \\ \hline
$\mL_{1}$      &  3 &  \\ \hline
$\mLa^{a}$     & 4 &  \multirow{3}{*}{$\bKSa{ \tau}$} \\ \cline{1-2}
$\mLa^{b}$     & 4 &  \\ \cline{1-2}
$\mLa^{c}$     & 1 & \\ \hline
$\mLb^{a}$     & 4 & $\bKSc{ \tau}$ \\ \cline{1-2}
$\mLb^{b}$     & 2 &  $\bKSb{ \tau,\taup}$ \\ \hline
\end{tabular}
}
\end{table}
